Sensitivity to millicharged particles in future proton-proton collisions at the LHC

We report on the expected sensitivity of dedicated scintillator-based detectors at the LHC for elementary particles with charges much smaller than the electron charge. The dataset provided by a prototype scintillator-based detector is used to characterise the performance of the detector and provide an accurate background projection. Detector designs, including a novel slab detector configuration, are considered for the data taking period of the LHC to start in 2022 (Run 3) and for the high luminosity LHC. With the Run 3 dataset, the existence of new particles with masses between 10 MeV and 45 GeV could be excluded at 95% confidence level for charges between 0.003e and 0.3e, depending on their mass. With the high luminosity LHC dataset, the expected limits would reach between 10 MeV and 80 GeV for charges between 0.0018e and 0.3e, depending on their mass

==> authorlist.tex <==

%
% SORTED BY LAST NAME
%
\author{A.~Ball}\affiliation{CERN, Geneva, Switzerland}
%\author{G.~Beauregard}\affiliation{New York University, New York, New York 10012, USA}
\author{J.~Brooke}\affiliation{University of Bristol, Bristol, United Kingdom}
\author{C.~Campagnari}\affiliation{University of California, Santa Barbara,  California 93106, USA}
\author{M.~Carrigan}\affiliation{The Ohio State University, Columbus, Ohio 43218, USA}
\author{M.~Citron}\affiliation{University of California, Santa Barbara,  California 93106, USA}
%\author{J.~De~La~Haye}\affiliation{CERN, Geneva, Switzerland}
\author{A.~De~Roeck}\affiliation{CERN, Geneva, Switzerland}
%\author{R.~Escobar~Franco}\affiliation{University of California, Santa Barbara,  California 93106, USA}
\author{M.~Ezeldine}\affiliation{Lebanese University, Hadeth-Beirut, Lebanon}
\author{B.~Francis}\affiliation{The Ohio State University, Columbus, Ohio 43218, USA}
\author{M.~Gastal}\affiliation{CERN, Geneva, Switzerland}
\author{M.~Ghimire}\affiliation{New York University, New York, New York 10012, USA}
\author{J.~Goldstein}\affiliation{University of Bristol, Bristol, United Kingdom}
\author{F.~Golf}\affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
%\author{J.~Guiang}\thanks{Now at University of California, San Diego, California 92093, USA.}\affiliation{University of California, Santa Barbara,  California 93106, USA}
\author{A.~Haas}\affiliation{New York University, New York, New York 10012, USA}
\author{R.~Heller}\thanks{Now at Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA.}\affiliation{University of California, Santa Barbara,  California 93106, USA}
\author{C.S.~Hill}\affiliation{The Ohio State University, Columbus, Ohio 43218, USA}
\author{L.~Lavezzo}\affiliation{The Ohio State University, Columbus, Ohio 43218, USA}
\author{R.~Loos}\affiliation{CERN, Geneva, Switzerland}
\author{S.~Lowette}\affiliation{Vrije Universiteit Brussel, Brussels, Belgium}
%\author{G.~Magill}\affiliation{McMaster University, Hamilton, Canada}\affiliation{Perimeter Institute for Theoretical Physics, Waterloo, Canada}
\author{B.~Manley}\affiliation{The Ohio State University, Columbus, Ohio 43218, USA}
\author{B.~Marsh}\affiliation{University of California, Santa Barbara,  California 93106, USA}
\author{D.W.~Miller}\affiliation{University of Chicago, Chicago, Illinois 60637, USA}
\author{B.~Odegard}\affiliation{University of California, Santa Barbara,  California 93106, USA}
%\author{F.R.~Saab}\affiliation{Lebanese University, Hadeth-Beirut, Lebanon}
%\author{J.~Sahili}\affiliation{Lebanese University, Hadeth-Beirut, Lebanon}
\author{R.~Schmitz}\affiliation{University of California, Santa Barbara,  California 93106, USA}
\author{F.~Setti}\affiliation{University of California, Santa Barbara,  California 93106, USA}
\author{H.~Shakeshaft}\affiliation{CERN, Geneva, Switzerland}
\author{D.~Stuart}\affiliation{University of California, Santa Barbara,  California 93106, USA}
\author{M.~Swiatlowski}\thanks{Now at TRIUMF, Vancouver, Canada.}\affiliation{University of Chicago, Chicago, Illinois 60637, USA}
\author{J.~Yoo}\thanks{Now at Korea University, Seoul, South Korea.}\affiliation{University of California, Santa Barbara,  California 93106, USA}
\author{H.~Zaraket}\affiliation{Lebanese University, Hadeth-Beirut, Lebanon}
%\author{H.~Zheng}\affiliation{University of Chicago, Chicago, Illinois 60637, USA}

